Temporal HAL-API Dependencies as a Gateway to Formal Embedded Software Development

Temporal HAL-API Dependencies (THADs) can be useful to capture an interesting class of correctness properties in embedded software development. They demand a moderate effort for specification (which can be done via program annotations) and verification (which can be done automatically via software model checking). In this sense, they have the potential to form an interesting sweet spot between generic properties (that demand virtually no specification effort, and that are typically addressed by static analysis) and application-specific properties as addressed by full-fledged formal methods. Thus, they may form a gateway to wider and more economic use of formal methods in industrial embedded software development.

==> macros.tex <==
% Define abbreviations including dots
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{e.g\onedot} \def\Eg{E.g\onedot}
\def\ie{i.e\onedot} \def\Ie{I.e\onedot}
\def\cf{c.f\onedot} \def\Cf{C.f\onedot}
\def\etc{etc\onedot}
\def\wrt{w.r.t\onedot}
\def\dof{d.o.f\onedot}
\def\vs{vs\onedot}
\def\etal{et al\onedot}
\makeatother

% Define macro to typeset overline text
\makeatletter
\newcommand{\textoverline}[1]{$\overline{\hbox{#1}}\m@th$}
\makeatother

% Define section names for \autoref{...} macro
\renewcommand{\sectionautorefname}{Section}
\renewcommand{\subsectionautorefname}{Subsection}
\renewcommand{\subsubsectionautorefname}{Subsection}

% Define macros for tool and hardware names
\newcommand{\trezor}{\emph{Trezor}\xspace}
\newcommand{\ultimate}{\textsc{Ultimate}\xspace}
\newcommand{\ultimateAutomizer}{\textsc{Ultimate Automizer}\xspace}
\newcommand{\raspberryPi}{Raspberry~Pi~3 Model~B+\xspace}
\newcommand{\spidev}{\textit{spidev}\xspace}

% Define macros for THADs
\newcommand{\opdep}{\triangleleft}
\newcommand{\varThad}{\delta}
\newcommand{\varThadDep}[3]{#1 : #2 \opdep #3}

% Define check- and cross mark
\newcommand{\cmark}{\checkmark}
\newcommand{\xmark}{\text{\ding{55}}}

% Define macros to typeset code and parameters
\newcommand{\code}[1]{\texttt{#1}\xspace}
\newcommand{\codeParam}[1]{\code{#1}}

% Define spidev HAL-API routines
\DeclareRobustCommand\Compactcdots{\mathinner{\ldotp\mkern-3mu\ldotp\mkern-3mu\ldotp}}
\newcommand\halDots{\ifmmode\ldots\else$\Compactcdots$\fi}

\newcommand{\fildes}{\code{fd}}
\newcommand{\rpiSpiDeviceFile}{/dev/spidev0.0}
\newcommand{\rpiSpiDeviceFileString}{"/dev/spidev0.0"}
\newcommand{\deviceFileRW}{O\_RDWR}

\newcommand{\halApiRoutineInit}{\code{init()}}
\newcommand{\halApiRoutineInitS}{\code{init}}
\newcommand{\halApiRoutineSend}{\code{send()}}
\newcommand{\halApiRoutineSendS}{\code{send}}
\newcommand{\halApiRoutineOpen}{\code{open()}}
\newcommand{\halApiRoutineOpenS}{\code{open}}
\newcommand{\halApiRoutineOpenD}{\code{open(\halDots)}}
\newcommand{\halApiRoutineOpenP}[2]{\code{open(\codeParam{#1},\,\codeParam{#2})}}
\newcommand{\halApiRoutineOpenF}[3]{\code{\codeParam{#1}\,:=\,open(\codeParam{#2},\,\codeParam{#3})}}
\newcommand{\halApiRoutineOpenDR}{\code{fd\,:=\,open(\halDots)}}
\newcommand{\halApiRoutineOpenPRpi}{\halApiRoutineOpenP{\rpiSpiDeviceFileString}{\deviceFileRW}}
\newcommand{\halApiRoutineOpenRpi}{\halApiRoutineOpenF{\fildes}{\rpiSpiDeviceFileString}{\deviceFileRW}}
\newcommand{\halApiRoutineClose}{\code{close()}}
\newcommand{\halApiRoutineCloseS}{\code{close}}
\newcommand{\halApiRoutineCloseF}{\code{close(\fildes)}}
\newcommand{\halApiRoutineRead}{\code{read()}}
\newcommand{\halApiRoutineReadS}{\code{read}}
\newcommand{\halApiRoutineReadF}{\code{read(\fildes)}}
\newcommand{\halApiRoutineReadFD}{\code{read(\fildes,\,\halDots)}}
\newcommand{\halApiRoutineWrite}{\code{write()}}
\newcommand{\halApiRoutineWriteS}{\code{write}}
\newcommand{\halApiRoutineWriteF}{\code{write(\fildes)}}
\newcommand{\halApiRoutineWriteFD}{\code{write(\fildes,\,\halDots)}}
\newcommand{\halApiRoutineIoctl}[1]{\code{ioctl(#1)}}
\newcommand{\halApiRoutineIoctlS}{\code{ioctl}}

\newcommand{\halApiRoutineParamValueMsg}{\codeParam{MSG}}
\newcommand{\halApiRoutineParamValueRWMode}{\codeParam{\{RD,WR\}\_MODE}}
\newcommand{\halApiRoutineParamValueRMode}{\codeParam{RD\_MODE}}
\newcommand{\halApiRoutineParamValueWMode}{\codeParam{WR\_MODE}}
\newcommand{\halApiRoutineParamValueRWModeExt}{\codeParam{\{RD,WR\}\_MODE32}}
\newcommand{\halApiRoutineParamValueRModeExt}{\codeParam{RD\_MODE32}}
\newcommand{\halApiRoutineParamValueWModeExt}{\codeParam{WR\_MODE32}}
\newcommand{\halApiRoutineParamValueRWLSBF}{\codeParam{\{RD,WR\}\_LSB\_FIRST}}
\newcommand{\halApiRoutineParamValueRLSBF}{\codeParam{RD\_LSB\_FIRST}}
\newcommand{\halApiRoutineParamValueWLSBF}{\codeParam{WR\_LSB\_FIRST}}
\newcommand{\halApiRoutineParamValueRWBitsPWord}{\codeParam{\{RD,WR\}\_BITS\_PER\_WORD}}
\newcommand{\halApiRoutineParamValueRBitsPWord}{\codeParam{RD\_BITS\_PER\_WORD}}
\newcommand{\halApiRoutineParamValueWBitsPWord}{\codeParam{WR\_BITS\_PER\_WORD}}
\newcommand{\halApiRoutineParamValueRWSpeed}{\codeParam{\{RD,WR\}\_MAX\_SPEED\_HZ}}
\newcommand{\halApiRoutineParamValueRSpeed}{\codeParam{RD\_MAX\_SPEED\_HZ}}
\newcommand{\halApiRoutineParamValueWSpeed}{\codeParam{WR\_MAX\_SPEED\_HZ}}

\newcommand{\halApiRoutineIoctlParamFildes}{\codeParam{fildes}}
\newcommand{\halApiRoutineIoctlParamRequest}{\codeParam{request}}
\newcommand{\halApiRoutineIoctlLiteralPrefix}{\codeParam{SPI\_IOC\_}}

\newcommand{\halApiRoutineIoctlMsg}{\halApiRoutineIoctl{\halApiRoutineParamValueMsg}}
\newcommand{\halApiRoutineIoctlMsgF}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueMsg}}
\newcommand{\halApiRoutineIoctlMsgFD}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueMsg,\,\halDots}}
\newcommand{\halApiRoutineIoctlRWMode}{\halApiRoutineIoctl{\halApiRoutineParamValueRWMode}}
\newcommand{\halApiRoutineIoctlRWModeF}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueRWMode}}
\newcommand{\halApiRoutineIoctlRWModeFD}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueRWMode,\,\halDots}}
\newcommand{\halApiRoutineIoctlRMode}{\halApiRoutineIoctl{\halApiRoutineParamValueRMode}}
\newcommand{\halApiRoutineIoctlRModeF}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueRMode}}
\newcommand{\halApiRoutineIoctlRModeFD}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueRMode,\,\halDots}}
\newcommand{\halApiRoutineIoctlWMode}{\halApiRoutineIoctl{\halApiRoutineParamValueWMode}}
\newcommand{\halApiRoutineIoctlWModeF}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueWMode}}
\newcommand{\halApiRoutineIoctlWModeFD}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueWMode,\,\halDots}}
\newcommand{\halApiRoutineIoctlRWModeExt}{\halApiRoutineIoctl{\halApiRoutineParamValueRWModeExt}}
\newcommand{\halApiRoutineIoctlRWModeExtF}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueRWModeExt}}
\newcommand{\halApiRoutineIoctlRWModeExtFD}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueRWModeExt,\,\halDots}}
\newcommand{\halApiRoutineIoctlRModeExt}{\halApiRoutineIoctl{\halApiRoutineParamValueRModeExt}}
\newcommand{\halApiRoutineIoctlRModeExtF}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueRModeExt}}
\newcommand{\halApiRoutineIoctlRModeExtFD}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueRModeExt,\,\halDots}}
\newcommand{\halApiRoutineIoctlWModeExt}{\halApiRoutineIoctl{\halApiRoutineParamValueWModeExt}}
\newcommand{\halApiRoutineIoctlWModeExtF}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueWModeExt}}
\newcommand{\halApiRoutineIoctlWModeExtFD}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueWModeExt,\,\halDots}}
\newcommand{\halApiRoutineIoctlRWLSBF}{\halApiRoutineIoctl{\halApiRoutineParamValueRWLSBF}}
\newcommand{\halApiRoutineIoctlRWLSBFF}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueRWLSBF}}
\newcommand{\halApiRoutineIoctlRWLSBFFD}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueRWLSBF,\,\halDots}}
\newcommand{\halApiRoutineIoctlRLSBF}{\halApiRoutineIoctl{\halApiRoutineParamValueRLSBF}}
\newcommand{\halApiRoutineIoctlRLSBFF}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueRLSBF}}
\newcommand{\halApiRoutineIoctlRLSBFFD}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueRLSBF,\,\halDots}}
\newcommand{\halApiRoutineIoctlWLSBF}{\halApiRoutineIoctl{\halApiRoutineParamValueWLSBF}}
\newcommand{\halApiRoutineIoctlWLSBFF}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueWLSBF}}
\newcommand{\halApiRoutineIoctlWLSBFFD}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueWLSBF,\,\halDots}}
\newcommand{\halApiRoutineIoctlRWBitsPWord}{\halApiRoutineIoctl{\halApiRoutineParamValueRWBitsPWord}}
\newcommand{\halApiRoutineIoctlRWBitsPWordF}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueRWBitsPWord}}
\newcommand{\halApiRoutineIoctlRWBitsPWordFD}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueRWBitsPWord,\,\halDots}}
\newcommand{\halApiRoutineIoctlRBitsPWord}{\halApiRoutineIoctl{\halApiRoutineParamValueRBitsPWord}}
\newcommand{\halApiRoutineIoctlRBitsPWordF}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueRBitsPWord}}
\newcommand{\halApiRoutineIoctlRBitsPWordFD}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueRBitsPWord,\,\halDots}}
\newcommand{\halApiRoutineIoctlWBitsPWord}{\halApiRoutineIoctl{\halApiRoutineParamValueWBitsPWord}}
\newcommand{\halApiRoutineIoctlWBitsPWordF}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueWBitsPWord}}
\newcommand{\halApiRoutineIoctlWBitsPWordFD}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueWBitsPWord,\,\halDots}}
\newcommand{\halApiRoutineIoctlRWSpeed}{\halApiRoutineIoctl{\halApiRoutineParamValueRWSpeed}}
\newcommand{\halApiRoutineIoctlRWSpeedF}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueRWSpeed}}
\newcommand{\halApiRoutineIoctlRWSpeedFD}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueRWSpeed,\,\halDots}}
\newcommand{\halApiRoutineIoctlRSpeed}{\halApiRoutineIoctl{\halApiRoutineParamValueRSpeed}}
\newcommand{\halApiRoutineIoctlRSpeedF}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueRSpeed}}
\newcommand{\halApiRoutineIoctlRSpeedFD}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueRSpeed,\,\halDots}}
\newcommand{\halApiRoutineIoctlWSpeed}{\halApiRoutineIoctl{\halApiRoutineParamValueWSpeed}}
\newcommand{\halApiRoutineIoctlWSpeedF}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueWSpeed}}
\newcommand{\halApiRoutineIoctlWSpeedFD}{\halApiRoutineIoctl{\fildes,\,\halApiRoutineParamValueWSpeed,\,\halDots}}

